Regressing Transformers for Data-efficient Visual Place Recognition

Visual place recognition is a critical task in computer vision, especially for localization and navigation systems. Existing methods often rely on contrastive learning: image descriptors are trained to have small distance for similar images and larger distance for dissimilar ones in a latent space. However, this approach struggles to ensure accurate distance-based image similarity representation, particularly when training with binary pairwise labels, and complex re-ranking strategies are required. This work introduces a fresh perspective by framing place recognition as a regression problem, using camera field-of-view overlap as similarity ground truth for learning. By optimizing image descriptors to align directly with graded similarity labels, this approach enhances ranking capabilities without expensive re-ranking, offering data-efficient training and strong generalization across several benchmark datasets.

==> sections/5_discussion.tex <==


In this section we elaborate on the effect of whitening and dimensionality reduction, the data efficiency of our methods, the quality of our learned features and of the attention maps of our models. Moreover, we study the effect of learning with a different metric.
\subsection{Whitening}
\label{sec:whitening}




